Learning Control Policies for Stochastic Systems with Reach-avoid Guarantees

We study the problem of learning controllers for discrete-time non-linear stochastic dynamical systems with formal reach-avoid guarantees. This work presents the first method for providing formal reach-avoid guarantees, which combine and generalize stability and safety guarantees, with a tolerable probability threshold $p\in[0,1]$ over the infinite time horizon. Our method leverages advances in machine learning literature and it represents formal certificates as neural networks. In particular, we learn a certificate in the form of a reach-avoid supermartingale (RASM), a novel notion that we introduce in this work. Our RASMs provide reachability and avoidance guarantees by imposing constraints on what can be viewed as a stochastic extension of level sets of Lyapunov functions for deterministic systems. Our approach solves several important problems -- it can be used to learn a control policy from scratch, to verify a reach-avoid specification for a fixed control policy, or to fine-tune a pre-trained policy if it does not satisfy the reach-avoid specification. We validate our approach on $3$ stochastic non-linear reinforcement learning tasks.

==> [AAAI 2023] Reach-avoid (2)/supplementary_for_arxiv2.tex <==
\begin{center}
	\Large\textbf{Appendix}
\end{center}

\section{Overview of Martingale Theory}\label{sec:martingales}

\paragraph{Probability theory} A {\em probability space} is a triple $(\Omega,\mathcal{F},\mathbb{P})$, where $\Omega$ is a non-empty {\em sample space}, $\mathcal{F}$ is a $\sigma$-algebra over $\Omega$ (i.e.~a collection of subsets of $\Omega$ that contains the empty set $\emptyset$ and is closed under complementation and countable union operations), and $\mathbb{P}$ is a {\em probability measure} over $\mathcal{F}$, i.e.~a function $\mathbb{P}:\mathcal{F}\rightarrow[0,1]$ that satisfies Kolmogorov axioms~\cite{Williams91}. We call the elements of $\mathcal{F}$ {\em events}. Given a probability space $(\Omega,\mathcal{F},\mathbb{P})$, a {\em random variable} is a function $X:\Omega\rightarrow\mathbb{R}$ that is $\mathcal{F}$-measurable, i.e.~for each $a\in\mathbb{R}$ we have that $\{\omega\in\Omega\mid X(\omega)\leq a\}\in\mathcal{F}$. We use $\mathbb{E}[X]$ to denote the {\em expected value} of $X$. A {\em (discrete-time) stochastic process} is a sequence $(X_i)_{i=0}^{\infty}$ of random variables in $(\Omega,\mathcal{F},\mathbb{P})$.
	
\paragraph{Conditional expectation} In order to formally define supermartingales, we need to introduce conditional expectation. Let $X$ be a random variable in a probability space $(\Omega,\mathcal{F},\mathbb{P})$. Given a sub-$\sigma$-algebra $\mathcal{F}'\subseteq\mathcal{F}$, a {\em conditional expectation} of $X$ given $\mathcal{F}'$ is an $\mathcal{F}'$-measurable random variable $Y$ such that, for each $A\in\mathcal{F}'$, we have 
\[ \mathbb{E}[X\cdot\mathbb{I}(A)]=\mathbb{E}[Y\cdot\mathbb{I}(A)].\]
The function $\mathbb{I}(A):\Omega\rightarrow \{0,1\}$ is an {\em indicator function} of $A$, defined via $\mathbb{I}(A)(\omega)=1$ if $\omega\in A$, and $\mathbb{I}(A)(\omega)=0$ if $\omega\not\in A$. Intuitively, conditional expectation of $X$ given $\mathcal{F}'$ is an $\mathcal{F}'$-measurable random variable that behaves like $X$ whenever its expected value is taken over an event in $\mathcal{F}'$. It is known that a conditional expectation of a random variable $X$ given $\mathcal{F}'$ exists if $X$ is real-valued and nonnegative~\cite{Williams91}. Moreover, for any two $\mathcal{F}'$-measurable random variables $Y$ and $Y'$ which are conditional expectations of $X$ given $\mathcal{F}'$, we have that $\mathbb{P}[Y= Y']=1$. Therefore, the conditional expectation is almost-surely unique and we may pick any such random variable as a canonical conditional expectation and denote it by $\mathbb{E}[X\mid \mathcal{F}']$.

\paragraph{Supermartingales} We are now ready to define supermartingales. Let $(\Omega,\mathcal{F},\mathbb{P})$ be a probability space and $(\mathcal{F}_i)_{i=0}^\infty$ be an increasing sequence of sub-$\sigma$-algebras in $\mathcal{F}$, i.e.~$\mathcal{F}_0\subseteq\mathcal{F}_1\subseteq\dots\subseteq\mathcal{F}$. A nonnegative {\em supermartingale} with respect to $(\mathcal{F}_i)_{i=0}^\infty$ is a stochastic process $(X_i)_{i=0}^{\infty}$ such that each $X_i$ is $\mathcal{F}_i$-measurable, and $X_i(\omega)\geq 0$ and $\mathbb{E}[X_{i+1}\mid\mathcal{F}_i](\omega) \leq X_i(\omega)$ hold for each $\omega\in\Omega$ and $i\geq 0$. Intuitively, the second condition says that the expected value of $X_{i+1}$ given the value of $X_i$ has to decrease, and this requirement is formally captured via conditional expectation.

We now present two results that will be key ingredients in the proof of Theorem~1. The first is Doob's Supermartingale Convergence Theorem (see~\cite{Williams91}, Section~11) which shows that every nonnegative supermartingale converges almost-surely to some finite value. The second theorem (see~\cite{Kushner14}, Theorem~7.1) provides a bound on the probability that the value of the supemartingale ever exceeds some threshold, and it will allow us to reason about both probabilistic reachability and safety. This is a less standard result from martingale theory, so we prove it below. In what follows, let $(\Omega,\mathcal{F},\mathbb{P})$ be a probability space and $(\mathcal{F}_i)_{i=0}^\infty$ be an increasing sequence of sub-$\sigma$-algebras in $\mathcal{F}$. 

\begin{theorem}[Supermartingale convergence theorem]\label{thm:convergence}
Let $(X_i)_{i=0}^{\infty}$ be a nonnegative supermartingale with respect to $(\mathcal{F}_i)_{i=0}^\infty$. Then, there exists a random variable $X_{\infty}$ in $(\Omega,\mathcal{F},\mathbb{P})$ to which the supermartingale converges to with probability $1$, i.e.~$\mathbb{P}[\lim_{i\rightarrow\infty}X_i=X_{\infty}]=1$.
\end{theorem}

\begin{theorem}\label{thm:bound}
Let $(X_i)_{i=0}^{\infty}$ be a nonnegative supermartingale with respect to $(\mathcal{F}_i)_{i=0}^\infty$. Then, for every $\lambda>0$, we have
\[ \mathbb{P}\Big[ \sup_{i\geq 0}X_i \geq \lambda \Big] \leq \frac{\mathbb{E}[X_0]}{\lambda}. \]
\end{theorem}

\begin{proof}
Fix $\lambda>0$. Define a stopping time $T:\Omega\rightarrow\mathbb{N}_0\cup\{\infty\}$ via $T = \inf_{i\in\mathbb{N}_0} \{X_i\geq \lambda\}$. Then, for each $n\in\mathbb{N}_0$, define a random variable
\[ X_{T\land n} = X_T\cdot\mathbb{I}(T \leq n) + X_n \cdot \mathbb{I}(T > n) \]
where $X_T$ is a random variable defined via $X_T(\omega)=X_{T(\omega)}(\omega)$ for each $\omega\in\Omega$, and $\mathbb{I}$ is again the indicator function that we defined in Section~\ref{sec:martingales}. It is a classical result from martingale theory that, for any $n\in\mathbb{N}_0$, we have $\mathbb{E}[X_{T\land n}]\leq \mathbb{E}[X_0]$ (see~\cite{Williams91}, Section 10.9). Hence, in order to prove the desired inequality, it suffices to prove $\lambda\cdot\mathbb{P}[ \sup_{i\geq 0}X_i \geq \lambda]\leq \sup_{n\in\mathbb{N}_0}\mathbb{E}[X_{T\land n}]$.

To prove the desired inequality we observe that, for each $n\in\mathbb{N}_0$, we have that
\begin{equation}\label{eq:stopping}
\begin{split}
    \mathbb{E}[X_{T\land n}] &= \mathbb{E}[X_T\cdot\mathbb{I}(T \leq n)] + \mathbb{E}[X_n \cdot \mathbb{I}(T > n)] \\
    &\geq \mathbb{E}[\lambda\cdot\mathbb{I}(T \leq n)] + \mathbb{E}[X_n \cdot \mathbb{I}(T > n)] \\
    &= \lambda\cdot\mathbb{P}[T \leq n] + \mathbb{E}[X_n \cdot \mathbb{I}(T > n)] \\
    &\geq \lambda\cdot\mathbb{P}[T \leq n] = \lambda\cdot\mathbb{P}[\sup_{0\leq i\leq n}X_i\geq \lambda].
\end{split}
\end{equation}
where in the first inequality we use the fact that $X_T\geq\lambda$, in the second inequality we use the fact that each $X_n$ is nonnegative and in the last equality we use the fact that $T = \inf_{i\in\mathbb{N}_0} \{X_i\geq \lambda\}$. Finally, $(\mathbb{P}[\sup_{0\leq i\leq n}X_i\geq \lambda])_{n=0}^\infty$ is a sequence of probabilities of events that are increasing with respect to set inclusion, so by the Monotone Convergence Theorem (see~\cite{Williams91}, Section 5.3) it follows that
\[ \lim_{n\rightarrow\infty}\mathbb{P}[\sup_{1\leq i\leq n}X_i\geq \lambda] = \mathbb{P}[\sup_{i\in\mathbb{N}_0}X_i\geq \lambda]. \]
Hence, by taking the supremum over $n\in\mathbb{N}_0$ of both sides of eq.~\eqref{eq:stopping}, we conclude that $\lambda\cdot\mathbb{P}[ \sup_{i\geq 0}X_i \geq \lambda]\leq \sup_{n\in\mathbb{N}_0}\mathbb{E}[X_{T\land n}]$, as desired. This concludes the proof of Theorem~\ref{thm:bound} since
\[ \mathbb{P}\Big[ \sup_{i\geq 0}X_i \geq \lambda \Big] \leq \sup_{n\in\mathbb{N}_0}\frac{\mathbb{E}[X_{T\land n}]}{\lambda} \leq \frac{\mathbb{E}[X_0]}{\lambda}. \]
\end{proof}

\section{Proof of Theorem~1}\label{sec:thmproof}

We now prove Theorem~1. Fix an initial state $\mathbf{x}_0\in\Init$ so that we need to show $\mathbb{P}_{\mathbf{x}_0}[ \ReachSafe(\Target,\Unsafe) ] \geq p$. Let $V$ be an RASM with respect to $\Target$, $\Unsafe$ and $p\in[0,1)$ whose existence is assumed in the theorem. First, we show that $V$ gives rise to a supermartingale in the probability space $(\Omega_{\mathbf{x}_0},\mathcal{F}_{\mathbf{x}_0},\mathbb{P}_{\mathbf{x}_0})$ of all trajectories of the system that start in $\mathbf{x}_0$. Then, we use Theorem~\ref{thm:convergence} and Theorem~\ref{thm:bound} to prove probabilistic reachability and safety.

For each time step $t\in\mathbb{N}_0$, define $\mathcal{F}_{\mathbf{x}_0,t}\subseteq\mathcal{F}_{\mathbf{x}_0}$ to be a sub-$\sigma$-algebra that, intuitively, contains events that are defined in terms of the first $t$ states of the system. Formally, for each $j\in\mathbb{N}_0$, let $C_j:\Omega_{\mathbf{x}_0}\rightarrow \mathcal{X}$ assign to each trajectory $\rho=(\mathbf{x}_t,\mathbf{u}_t,\omega_t)_{t\in\mathbb{N}_0}\in\Omega_{\mathbf{x}_0}$ the $j$-th state $\mathbf{x}_j$ along the trajectory. We define $\mathcal{F}_i$ to be the smallest $\sigma$-algebra over $\Omega_{\mathbf{x}_0}$ with respect to which $C_0, C_1, \dots, C_i$ are all measurable, where $\mathcal{X}\subseteq\mathbb{R}^m$ is equipped with the induced subset Borel-$\sigma$-algebra. The sequence $(\mathcal{F}_{\mathbf{x}_0,t})_{t=0}^\infty$ is increasing with respect to set inclusion.

Now, define a stochastic process $(X_t)_{t=0}^\infty$ in the probability space $(\Omega_{\mathbf{x}_0},\mathcal{F}_{\mathbf{x}_0},\mathbb{P}_{\mathbf{x}_0})$ via
\begin{equation*}
X_t(\rho) = \begin{cases}
    V(\mathbf{x}_t), &\text{if } \mathbf{x}_i\not\in\Target \text{ and } V(\mathbf{x}_i) < \frac{1}{1-p}\\
    &\text{for each } 0\leq i \leq t\\
    0, &\text{if } \mathbf{x}_i\in\Target \text{ for some }0\leq i\leq t \text{ and}\\
    &V(\mathbf{x}_j) < \frac{1}{1-p} \text{ for each }0\leq j\leq i\\
    \frac{1}{1-p}, &\text{otherwise}
\end{cases}
\end{equation*}
for each $t\in\mathbb{N}_0$ and a trajectory $\rho=(\mathbf{x}_t,\mathbf{u}_t,\omega_t)_{t\in\mathbb{N}_0}$. In other words, the value of $X_t$ is equal to the value of $V$ at $\mathbf{x}_t$, unless either the target set $\Target$ has been reached first in which case we set all future values of $\mathcal{X}_t$ to $0$, or a state in which $V$ exceeds $\frac{1}{1-p}$ has been reached first in which case we set all future values of $\mathcal{X}_t$ to $\frac{1}{1-p}$. We claim that $(X_t)_{t=0}^\infty$ is a nonnegative supermartingale with respect to $(\mathcal{F}_{\mathbf{x}_0,t})_{t=0}^\infty$. Indeed, each $X_t$ is $\mathcal{F}_{\mathbf{x}_0,t}$-measurable as it is defined in terms of the first $t$ states along a trajectory. It is also nonnegative as $V$ is nonnegative by the Nonnegativity condition of RASMs. Finally, to see that $\mathbb{E}_{\mathbf{x}_0}[X_{t+1}\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho) \leq X_t(\rho)$ holds for each $t\in\mathbb{N}_0$ and $\rho=(\mathbf{x}_t,\mathbf{u}_t,\omega_t)_{t\in\mathbb{N}_0}$, we consider $3$ cases:
\begin{enumerate}
    \item If $\mathbf{x}_0,\mathbf{x}_1,\dots,\mathbf{x}_t\not\in\Target$ and $V(\mathbf{x}_i) < \frac{1}{1-p}$ for each $0\leq i\leq t$, then
    \begin{equation*}
    \begin{split}
        &\mathbb{E}_{\mathbf{x}_0}[X_{t+1}\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho) \\
        &= \mathbb{E}_{\mathbf{x}_0}\Big[X_{t+1}\cdot \Big(\mathbb{I}(\mathbf{x}_{t+1}\not\in\Target \land V(\mathbf{x}_{t+1})<\frac{1}{1-p}) \\
        &\,\,\,+ \mathbb{I}(\mathbf{x}_{t+1}\in\Target) + \mathbb{I}(V(\mathbf{x}_{t+1})\geq \frac{1}{1-p})\Big)\mid\mathcal{F}_{\mathbf{x}_0,t}\Big](\rho) \\
        &= \mathbb{E}_{\mathbf{x}_0}[X_{t+1}\cdot \mathbb{I}(\mathbf{x}_{t+1}\not\in\Target)\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho) \\
        &\,\,\,+ 0 + \frac{1}{1-p}\cdot\mathbb{E}[\mathbb{I}(V(\mathbf{x}_{t+1})\geq \frac{1}{1-p})\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho)
    \end{split}
    \end{equation*}
    \begin{equation*}
    \begin{split}
        &\leq \mathbb{E}_{\omega\sim d}[V(f(\mathbf{x}_t,\mathbf{u}_t,\omega_t))\cdot\mathbb{I}(\mathbf{x}_{t+1}\not\in\Target \land V(\mathbf{x}_{t+1})<\frac{1}{1-p})] \\
        &\,\,\,+ \mathbb{E}_{\omega\sim d}[V(f(\mathbf{x}_t,\mathbf{u}_t,\omega_t))\cdot\mathbb{I}(\mathbf{x}_{t+1}\in\Target)] \\
        &\,\,\,+ \mathbb{E}_{\omega\sim d}[V(f(\mathbf{x}_t,\mathbf{u}_t,\omega_t))\cdot\mathbb{I}(V(\mathbf{x}_{t+1})\geq\frac{1}{1-p})] \\
        &= \mathbb{E}_{\omega\sim d}[V(f(\mathbf{x}_t,\mathbf{u}_t,\omega_t))] \\
        &\leq V(\mathbf{x}_t) - \eps.
    \end{split}
    \end{equation*}
    Here, the first equality follows by the law of total probability, the second equality follows by our definition of each $X_t$, the third inequality follows by observing that $V(\mathbf{x}_{t+1})\geq X_{t+1}(\rho)$ in this case, the fourth equality is just the sum of expectations over disjoint sets, and finally the fifth inequality follows by the Expected decrease condition in Definition~1 since $\mathbf{x}_t\not\in\Target$ and $V(\mathbf{x}_t)<\frac{1}{1-p}$, by the assumption of this case.
    
    \item If $\mathbf{x}_i\in\Target$ for some $0\leq i\leq t$ and $V(\mathbf{x}_j)<\frac{1}{1-p}$ for all $0\leq j\leq i$, then we have $\mathbb{E}_{\mathbf{x}_0}[X_{t+1}\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho)=X_{t+1}(\rho)=0$.
    
    \item Otherwise, we must have $V(\mathbf{x}_i)\geq\frac{1}{1-p}$ and $\mathbf{x}_0,\dots,\mathbf{x}_i\not\in\Target$ for some $-\leq i\leq t$, thus $\mathbb{E}_{\mathbf{x}_0}[X_{t+1}\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho)=X_{t+1}(\rho)=\frac{1}{1-p}$.
\end{enumerate}
Hence, we have proved that $(X_t)_{t=0}^\infty$ is a nonnegative supermartingale.

Now, by Theorem~\ref{thm:convergence} it follows that the value of the nonnegative supermartingale $(X_t)_{t=0}^\infty$ with probability $1$ converges. In what follows, we show that $(X_t)_{t=0}^\infty$ with probability $1$ converges to and reaches either $0$ or a value that is greater than or equal to $\frac{1}{1-p}$. To do this, we use the fact that the Expected decrease condition of RASMs enforces the value of $V$ to decrease in expected value by at least $\eps>0$ after every one-step evolution of the system in any non-target state at which $V(\mathbf{x}) < \frac{1}{1-p}$. Define the stopping time $T:\Omega_{\mathbf{x}_0}\rightarrow\mathbb{N}_0\cup\{\infty\}$ via
\[ T(\rho)=\inf_{t\in\mathbb{N}_0}\Big\{X_t(\rho)=0\lor X_t(\rho)\geq\frac{1}{1-p}\Big\}. \]
Our goal is then to prove that $\mathbb{P}_{\mathbf{x}_0}[T < \infty] = 1$. Using the argument in the proof that $(X_t)_{t=0}^{\infty}$ is a nonnegative supermartingale (in particular, the proof of supermartingale property in Case~$1$), we can in fact deduce a stronger inequality
\[ \mathbb{E}_{\mathbf{x}_0}[X_{t+1}\mid\mathcal{F}_{\mathbf{x}_0,t}](\rho)\leq X_t(\rho) - \eps\cdot \mathbb{I}(T(\rho) > t) \]
for each $\rho\in\Omega_{\mathbf{x}_0}$. But now, we may use Proposition~\ref{prop:convergence} stated below to deduce that $\mathbb{E}_{\mathbf{x}_0}[T]\leq \mathbf{E}_{\mathbf{x}_0}[X_0]=V(\mathbf{x}_0)<\infty$, which in turn implies that $\mathbb{P}_{\mathbf{x}_0}[T < \infty] = 1$, as desired. This concludes the proof.

The following proposition states a results on probability $1$ convergence of {\em ranking supermartingales (RSMs)}. RSMs are a notion similar to our RASMs that were first introduced in~\cite{ChakarovS13} in order to study termination in probabilistic programs, and were used in~\cite{lechner2021stability} to formally verify almost-sure stability and reachability in stochastic control systems. We note that RASMs generalize RSMs in the sense that RSMs coincide with RASMs in the special case when the unsafe set is empty and we only consider a probability~$1$ reachability specification, i.e.~$\Unsafe=\emptyset$.

\begin{proposition}[\cite{ChakarovS13}]\label{prop:convergence}
Let $(\Omega,\mathcal{F},\mathbb{P})$ be a probability space, let $(\mathcal{F}_i)_{i=0}^\infty$ be an increasing sequence of sub-$\sigma$-algebras in $\mathcal{F}$ and let $T$ be a stopping time with respect to $(\mathcal{F}_i)_{i=0}^\infty$. Suppose that $(X_i)_{i=0}^{\infty}$ is a stochastic process such that each $X_i$ is nonnegative and we have that 
\[ \mathbb{E}[X_{i+1}\mid\mathcal{F}_i](\omega)\leq X_i(\omega) - \eps\cdot \mathbb{I}(T(\omega) > i) \]
holds for each $i\in\mathbb{N}_0$ and $\omega\in\Omega$. Then $\mathbb{P}[T<\infty]=1$.
\end{proposition}

%On the other hand, by the Expected decrease condition of RASMs, we know that the value of $V$ decreases in expected value by at least $\eps>0$ after every one-step evolution of the system in any non-target state at which $V(\mathbf{x}) < \frac{1}{1-p}$. Due to strict decrease that is bounded from below by $\eps>0$, the value of $V$ and therefore of each $X_t$ must be strictly positive in each non-target state, while the value of each $X_t$ is equal to $0$ upon reaching the target set. Hence, we may show that $(X_t)_{t=0}^\infty$ with probability $1$ converges either to $0$ or to a value that is greater than or equal to $\frac{1}{1-p}$, as for any other value $X_t$ would need to decrease by at least $\eps>0$ in the next one-step evolution of the system. Furthermore, this value has to be {\em reached} due to the strict $\eps>0$ decrease. Formal proof of the last two claims is deferred to Appendix~\ref{app:thm1proof}.
%But we showed above that the system reaches a state at which $V(\mathbf{x})\geq \frac{1}{1-p}$ with probability at most $1-p$. Hence, with probability at least $p$ the system will reach the target set $\Target$without reaching the unsafe set $\Unsafe$, i.e.~we conclude that $\mathbb{P}_{\mathbf{x}_0}[ \ReachSafe(\Target,\Unsafe) ] \geq p$.

Finally, by using Theorem~\ref{thm:bound} for the nonnegative supermartingale $(X_t)_{t=0}^\infty$ and $\lambda=\frac{1}{1-p}>0$, it follows that $\mathbb{P}_{\mathbf{x}_0}[ \sup_{i\geq 0}X_i \geq \frac{1}{1-p} ] \leq (1-p)\cdot \mathbb{E}_{\mathbf{x}_0}[X_0] \leq 1-p$. The second inequality follows since $X_0(\rho) = V(\mathbf{x}_0)\leq 1$ for every $\rho\in\Omega_{\mathbf{x}_0}$ by the Initial condition of RASMs. Hence, as $(X_t)_{t=0}^\infty$ with probability $1$ either reaches $0$ or a value that is greater than or equal to $\frac{1}{1-p}$, we conclude that $(X_t)_{t=0}^\infty$ reaches $0$ without reaching a value that is greater than or equal to $\frac{1}{1-p}$ with probability at least $p$. By the definition of each $X_t$ and by the Safety condition of RASMs, this implies that with probability at least $p$ the system will reach the target set $\Target$without reaching the unsafe set $\Unsafe$, i.e.~that $\mathbb{P}_{\mathbf{x}_0}[ \ReachSafe(\Target,\Unsafe) ] \geq p$.

\section{Computation of Expected Values of Neural Networks}\label{sec:expvalcomputation}

We now describe the method for bounding the expected value of a neural network function over a given probability distribution. Let $\mathbf{x}\in\mathcal{X}$ be a fixed state, and suppose that we want to bound the expected value $\mathbb{E}_{\omega\sim d}[ V ( f(\mathbf{x}, \pi(\mathbf{x}), \omega) )]$. We partition the disturbance space $\mathcal{N}\subseteq\mathbb{R}^p$ into finitely many cells $\text{cell}(\mathcal{N}) = \{\mathcal{N}_1,\dots,\mathcal{N}_{k}\}$.
Let $\mathrm{maxvol}=\max_{\mathcal{N}_i\in \text{cell}(\mathcal{N})}\mathsf{vol}(\mathcal{N}_i)$ denote the maximal volume of any cell in the partition (with respect to the Lebesgue measure). The expected value is bounded via
%We say that the {\em mesh} of $\text{cell}(\mathcal{N})$ is the maximal volume with respect to the Lebesgue measure over $\mathbb{R}^p$ of any cell in the partition, i.e.~$\max_{\mathcal{N}_i\in \text{cell}(\mathcal{N})}\mathsf{vol}(\mathcal{N}_i)$. The algorithm then bounds the expected value via
\begin{equation*}
    \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\mathbf{x}, \pi(\mathbf{x}), \omega) \Big) \Big] \leq \sum_{\mathcal{N}_i\in \text{cell}(\mathcal{N})} \mathrm{maxvol} \cdot \sup_{\omega\in \mathcal{N}_i} F(\omega)
\end{equation*}
%\begin{equation*}
%\begin{split}
%    \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\mathbf{x}, \pi(\mathbf{x}), \omega) \Big) \Big] &\leq \sum_{\mathcal{N}_i\in \text{cell}(\mathcal{N})} \mathsf{vol}(\mathcal{N}_i) \cdot \sup_{\omega\in \mathcal{N}_i} F(\omega) \\
%    &\leq \sum_{\mathcal{N}_i\in \text{cell}(\mathcal{N})} \text{mesh} \cdot \sup_{\omega\in \mathcal{N}_i} F(\omega)
%\end{split}
%\end{equation*}
where $F(\omega) = V( f(\mathbf{x}, \pi(\mathbf{x}), \omega))$. Each supremum is then bounded from above via interval arithmetic by using the method of~\cite{Gowal18}. Note that $\mathrm{maxvol}$ is not finite if $\mathcal{N}$ is unbounded. In order to allow expected value computation for an unbounded $\mathcal{N}$ under the assumption that $d$ is a product of univariate distributions, the method first applies the probability integral transform~\cite{Murphy12} to each univariate probability distribution in $d$ in order to reduce the problem to the case of a probability distribution of bounded support.

\section{Proof of Theorem~2}\label{sec:proofthmverifier}

Suppose that the verifier verifies that $V$ satisfies eq.~(1) for each $\tilde{\mathbf{x}}\in\tilde{\mathcal{X}_e}$, eq.~(2) for each $\text{cell}\in \text{Cells}_{\Init}$ and eq.~(3) for each $\text{cell}\in \text{Cells}_{\Unsafe}$. The fact that the Initial and the Unsafe conditions in Definition~1 of RASMs are satisfied by $V$ then follows from the correctness of interval arithmetic abstract interpretation (IA-AI) of~\cite{Gowal18}. Thus, we only need to show that $V$ satisfies the Expected decrease condition in Definition~1.

%First, we show that $V$ satisfies the Initial condition, i.e.~that $V(\mathbf{x})\leq 1$ for all $\mathbf{x}\in\Init$. Indeed, fix $\mathbf{x}\in\Init$ and let $\tilde{\mathbf{x}}$ be a point in $\tilde{\Init}$ such that $||\mathbf{x}-\tilde{\mathbf{x}}||_1<\tau$. By construction, the set $\tilde{\Init}$ contains vertices of each discretization cell that intersects $\Init$, hence such $\tilde{\mathbf{x}}$ exists. We then have
%\begin{equation*}
%\begin{split}
%    &V(\mathbf{x}) \leq V(\tilde{\mathbf{x}}) + |V(\mathbf{x}) - V(\tilde{\mathbf{x}})| \\
%    &\leq 1 - L_V\cdot\tau + |V(\mathbf{x}) - V(\tilde{\mathbf{x}})| \leq 1,
%\end{split}
%\end{equation*}
%as desired. The first inequality follows by triangle inequality, the second inequality follows from eq.~(\ref{eq:initialstricter}) at $\tilde{\mathbf{x}}$, and the third inequality follows by the definition of Lipschitz constant and since $||\mathbf{x}-\tilde{\mathbf{x}}||_1<\tau$.

%Second, we show that $V$ satisfies the Unsafe condition, i.e.~that $V(\mathbf{x})\geq \frac{1}{1-p}$ for all $\mathbf{x}\in\Unsafe$. Fix $\mathbf{x}\in\Unsafe$ and let $\tilde{\mathbf{x}}$ be a point in $\tilde{\Unsafe}$ such that $||\mathbf{x}-\tilde{\mathbf{x}}||_1<\tau$. By construction, the set $\tilde{\Unsafe}$ contains vertices of each discretization cell that intersects $\Unsafe$, hence such $\tilde{\mathbf{x}}$ exists. We then have
%\begin{equation*}
%\begin{split}
%    &V(\mathbf{x}) \geq V(\tilde{\mathbf{x}}) - |V(\mathbf{x}) - V(\tilde{\mathbf{x}})| \\
%    &\geq \frac{1}{1-p} + L_V\cdot\tau - |V(\mathbf{x}) - V(\tilde{\mathbf{x}})| \geq 1,
%\end{split}
%\end{equation*}
%as desired. The first inequality follows by triangle inequality, the second inequality follows from eq.~(\ref{eq:unsafestricter}) at $\tilde{\mathbf{x}}$, and the third inequality follows by the definition of Lipschitz constant and since $||\mathbf{x}-\tilde{\mathbf{x}}||_1<\tau$.

To show that $V$ satisfies the Expected decrease condition, we need to show that there exists $\eps>0$ such that $V(\mathbf{x}) \geq \mathbb{E}_{\omega\sim d}[V(f(\mathbf{x},\pi(\mathbf{x}),\omega))] + \eps$ holds for all $\mathbf{x}\in\mathcal{X}\backslash\Target$ at which $V(\mathbf{x}) \leq \frac{1}{1-p}$.  We prove that $\eps>0$ defined via
\[ \eps = \min_{\tilde{\mathbf{x}}\in \tilde{\mathcal{X}_\eps}} \Big( V(\tilde{\mathbf{x}}) - \tau \cdot K - \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \Big) \]
satisfies this property. Note that $\eps>0$, as each $\tilde{\mathbf{x}}\in\tilde{\mathcal{X}_e}$ satisfies eq.~(1).

To show this, fix $\mathbf{x}\in\mathcal{X}\backslash\Target$ with $V(\mathbf{x})\leq \frac{1}{1-p}$ and let $\tilde{\mathbf{x}}\in\tilde{\mathcal{X}_e}$ be such that $||\mathbf{x}-\tilde{\mathbf{x}}||_1 \leq \tau$. By construction, the set $\tilde{\mathcal{X}_e}$ contains vertices of each discretization cell that intersects $\mathcal{X}\backslash\Target$ and that contains at least one state at which $V$ is less than or equal to $\frac{1}{1-p}$, hence such $\tilde{\mathbf{x}}$ exists. We then have
\begin{equation}\label{eq:long}
\begin{split}
    &\mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\mathbf{x}, \pi(\mathbf{x}), \omega) \Big) \Big] \\
    &\leq \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \\
    &\hspace{1cm}+ ||f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) - f(\mathbf{x}, \pi(\mathbf{x}), \omega)||_1 \cdot L_V \\
    &\leq \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \\
    &\hspace{1cm}+ ||(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) - (\mathbf{x}, \pi(\mathbf{x}), \omega)||_1 \cdot L_V\cdot L_f \\
    &\leq \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \\
    &\hspace{1cm}+ ||\tilde{\mathbf{x}} - \mathbf{x}||_1 \cdot L_V\cdot L_f \cdot (1 + L_{\pi}) \\
    &\leq \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \\
    &\hspace{1cm}+ \tau \cdot L_V\cdot L_f \cdot (1 + L_{\pi}).
\end{split}
\end{equation}
On the other hand, we also have
\begin{equation}\label{eq:short}
    V(\mathbf{x}) \geq V(\tilde{\mathbf{x}}) - ||\tilde{\mathbf{x}} - \mathbf{x}||_1 \cdot L_V \geq V(\tilde{\mathbf{x}}) - \tau\cdot L_V.
\end{equation}
Combining eq.(\ref{eq:long}) and (\ref{eq:short}), we conclude that
\begin{equation}
\begin{split}
    &V(\mathbf{x}) - \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\mathbf{x}, \pi(\mathbf{x}), \omega) \Big) \Big] \\
    &\geq V(\tilde{\mathbf{x}}) - \tau\cdot L_V - \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \\
    &\hspace{1cm}- \tau \cdot L_V\cdot L_f \cdot (1 + L_{\pi}) \\
    &= V(\tilde{\mathbf{x}}) - \tau\cdot K - \mathbb{E}_{\omega\sim d}\Big[ V \Big( f(\tilde{\mathbf{x}}, \pi(\tilde{\mathbf{x}}), \omega) \Big) \Big] \\
    &\geq \eps
\end{split}
\end{equation}
where the equality in the second last row follows by the definition of $K$, and the inequality in the last row follows by our choice of $\eps$. Hence, $V$ satisfies the Expected decrease condition and is indeed an RASM as in Definition~1.

\section{Auxiliary Loss Term}\label{sec:appauxiliary}

The loss term $\loss_{\text{Aux}}(\nu)$ is an auxiliary loss term that does not enforce any of the defining conditions of RASMs, however it is used to guide the learner towards a candidate that attains the global minimum in a state that is contained within the target set $\Target$. We empirically observed that this term prevents the updated policy from diverging from its objective to stabilize the system. It is defined via
\begin{equation*}
\begin{split}
    \loss_{\text{Aux}}(\nu) & = \max\{V_\nu (\hat{\mathbf{x}}_{\text{Target}})- \varepsilon,0 \} \\
    &+ \max\{\min_{\mathbf{x} \in \tilde{X}\cap \Target} V_\nu(\mathbf{x}) - \min_{\mathbf{x} \in C_{\text{init}}} V_\nu(\mathbf{x}),0 \} \\
    &+ \max\{\min_{\mathbf{x} \in \tilde{X}\cap \Target} V_\nu(\mathbf{x}) - \min_{\mathbf{x} \in C_{\text{unsafe}}} V_\nu(\mathbf{x}),0 \}
\end{split}
\end{equation*}
with $\tilde{\mathbf{x}}_{\text{Target}}$ being some state contained in the target set $\Target$ and $\varepsilon\geq 0$ an algorithm parameter.

\section{Proof of Theorem~3}\label{sec:proofthmlearner}

Suppose that $V_{\nu}$ satisfies eq.~(1) for each $\tilde{\mathbf{x}}\in\tilde{\mathcal{X}_e}$, eq.~(2) for each $\text{cell}\in \text{Cells}_{\Init}$ and eq.~(3) for each $\text{cell}\in \text{Cells}_{\Unsafe}$. Suppose that Lipschitz constants of $\pi_{\theta}$ and $V_{\nu}$ are below the thresholds specified by $\loss_{\text{Lipschitz}}(\theta)$ and $\loss_{\text{Lipschitz}}(\nu)$ and that the samples in $\loss_{\text{Decrease}}(\theta,\nu)$ are independent. We need to show that $\lim_{N\rightarrow \infty} \loss(\theta,\nu) = 0$ with probability $1$.

Since Lipschitz constants of $\pi_{\theta}$ and $V_{\nu}$ are below the thresholds specified by $\loss_{\text{Lipschitz}}(\theta)$ and $\loss_{\text{Lipschitz}}(\nu)$, we have that $\lambda\cdot (\loss_{\text{Lipschitz}}(\theta) + \loss_{\text{Lipschitz}}(\nu)) = 0$. Moreover, our initialization of $C_{\text{init}}$ and our design of the verifier module ensure that $C_{\text{init}}$ contains only states in $\Init$, hence $\loss_{\text{Init}}(\nu)=0$ as $V_{\nu}$ satisfies the Initial condition of RASMs. Note, $V_{\nu}$ satisfies all conditions checked by the verifier, hence by Theorem~2 we know that it is an RASM.  Similarly, $C_{\text{unsafe}}$ contains only states in $\Unsafe$, hence $\loss_{\text{Unsafe}}(\nu)=0$ as $V_{\nu}$ satisfies the Safety condition of RASMs. Thus, under theorem assumptions we have that
\begin{equation*}
\begin{split}
    &\loss(\theta,\nu) = \loss_{\text{Decrease}}(\theta,\nu) \\
    &= \frac{1}{|C_{\text{decrease}}|}\sum_{\mathbf{x}\in C_{\text{decrease}}} \Big( \max \\
    &\Big\{ \sum_{\omega_1,\dots, \omega_N \sim \mathcal{N}}\frac{V_{\nu}\big(f(\mathbf{x},\pi_\theta(\mathbf{x}),\omega_i)\big)}{N} -  V_{\theta}(\mathbf{x})  + \tau \cdot K, 0\Big\} \Big)
\end{split}
\end{equation*}

Hence, in order to prove that $\lim_{N\rightarrow \infty} \loss(\theta,\nu) = 0$ with probability $1$, it suffices to prove that for each $\mathbf{x}\in C_{\text{decrease}}$ with probability $1$ we have
\begin{equation*}
\begin{split}
    &\lim_{N\rightarrow\infty}\max\Big\{ \sum_{\omega_1,\dots, \omega_N \sim \mathcal{N}}\frac{V_{\nu}\big(f(\mathbf{x},\pi_\theta(\mathbf{x}),\omega_i)\big)}{N} \\
    &-  V_{\theta}(\mathbf{x}) + \tau \cdot K, 0\Big\} = 0.
\end{split}
\end{equation*}

The above sum is the mean of $N$ independently sampled successor states of $\mathbf{x}$, which are sampled according to the probability distribution defined by the system dynamics and the probability distribution $d$ over disturbance vectors. Since the state space of the system is assumed to be compact and $V_{\theta}$ is continuous as it is a neural network, the random value defined by the value of $V$ at a sampled successor state is bounded and therefore admits a well-defined and finite first moment. The Strong Law of Large Numbers~\cite{Williams91} then implies that the above sum converges to the expected value of this distribution as $N\rightarrow\infty$. Thus, with probability $1$, we have that\begin{equation*}
\begin{split}
    &\lim_{N\rightarrow\infty}\max\Big\{ \sum_{\omega_1,\dots, \omega_N \sim \mathcal{N}}\frac{V_{\nu}\big(f(\mathbf{x},\pi_\theta(\mathbf{x}),\omega_i)\big)}{N} -  V_{\theta}(\mathbf{x}) + \tau \cdot K, 0\Big\} \\
    &=\max\Big\{ \lim_{M\rightarrow\infty}\sum_{\omega_1,\dots, \omega_N \sim \mathcal{N}}\frac{V_{\nu}\big(f(\mathbf{x},\pi_\theta(\mathbf{x}),\omega_i)\big)}{N} -  V_{\theta}(\mathbf{x}) + \tau \cdot K, 0\Big\} \\
    &=\max\Big\{ \lim_{M\rightarrow\infty}\mathbb{E}_{\omega\sim d}\Big[f(\mathbf{x},\pi_\theta(\mathbf{x}),\omega)\big] -  V_{\theta}(\mathbf{x}) + \tau \cdot K, 0\Big\} \\
    &= 0.
\end{split}
\end{equation*}
The first equality holds since a limit may be interchanged with the maximum function over a finite number of arguments, the second equality holds with probability $1$ by the Strong Law of Large Numbers, and the third equality holds since $V_{\nu}$ satisfies eq.~(1) for each $\tilde{\mathbf{x}}\in\tilde{\mathcal{X}_e}$ and we have $C_{\text{decrease}}\subseteq \tilde{\mathcal{X}_e}$. This concludes our proof that $\lim_{N\rightarrow \infty} \loss(\theta,\nu) = 0$ with probability~$1$.

\section{Experiment details}\label{supp:experiment}
The dynamics of the 2D system is given by
\begin{equation}
     \mathbf{x}_{t+1} = \begin{pmatrix} 1 & 0.045 \\ 0 & 0.9 \end{pmatrix} \mathbf{x}_t + \begin{pmatrix} 0.45 \\0.5 \end{pmatrix} g(\mathbf{u}_t) + \begin{pmatrix}0.01 & 0 \\0 & 0.005 \end{pmatrix}  \omega, 
\end{equation}
with $\omega$ being the disturbance vector and $\omega[1],\omega[2] \sim \text{Triangular}$. Square brackets indicate the coordinate index, e.g.~$\omega[1]$ is the first coordinate of $\omega\in\mathbb{R}^2$. The probability density function of $\text{Triangular}$ is defined by 
\begin{equation}
    \text{Triangular}(x) := \begin{cases} 0 & \text{if } x< -1\\ 1 - |x| & \text{if } -1 \leq x \leq 1\\ 0 & \text{otherwise}\end{cases}.
\end{equation}
The function $g$ is defined as $g(u) = \max(\min(u,1),-1)$.
The state space of the 2D system is define as $\mathcal{X} = [-1.5,1.5]^2$. We define the target set as $\Target = [-0.2,0.2]^2$, the initial set $\Init = [-0.25,-0.2]\times [-0.1,0.1] \cup  [0.25,0.2]\times [-0.1,0.1] $ and the unsafe set $\Unsafe = [-1.5,-1.4]\times[-1.5,0] \cup  [1.4,1.5]\times[0,1.5]$.


For the inverted pendulum task, the dynamics is given by 
\begin{align*}
    \mathbf{x}_{t+1}[2] &:= (1-b)  \mathbf{x}_{t}[2] \\
    &+ \Delta \cdot \big( \frac{-1.5 \cdot G \cdot \text{sin}(\mathbf{x}_{t}[1]+\pi)}{2l} + \frac{3}{m l^2} 2g(\mathbf{u}_t)\big)\\
    &+ 0.02 \omega[1]\\
    \mathbf{x}_{t+1}[1] &:=  \mathbf{x}_{t}[1] + \Delta \cdot \mathbf{x}_{t+1}[2] + 0.01 \omega[2],
\end{align*}
with $\delta, G, m, l, b$ being defined in Table \ref{tab:invpend}.
The state space of the inverted pendulum environment is define as $\mathcal{X} = [-0.7,0.7]^2$. We define the target set as $\Target = [-0.2,0.2]^2$, the initial set $\Init = [-0.3,0.3]^2$ and the unsafe set $\Unsafe = [-0.7,-0.6]\times[-0.7,0] \cup  [0.6,0.7]\times[0,0.7]$.

\begin{table}[]
    \centering
    \begin{tabular}{c|c}\toprule
        Parameter & Value  \\\midrule
        $\Delta$ &  0.05\\
        $G$ & 10\\
        $m$ & 0.15\\
        $l$ & 0.5\\
        $b$ & 0.1\\\bottomrule
    \end{tabular}
    \caption{Parameters of the inverted pendulum task.}
    \label{tab:invpend}
\end{table}

The dynamics of the collision avoidance task is given by 
\begin{align*}
    d_1 & = \max\{0.33 ||\mathbf{x}_t - \begin{pmatrix}0\\ 1\end{pmatrix}|| ,0\}\\
    d_2 & = \max\{0.33 ||\mathbf{x}_t - \begin{pmatrix}0 \\-1\end{pmatrix}|| ,0\}\\
    \mathbf{x}_{t+1} & = \mathbf{x}_{t} + 0.2 \Big(d_2 \big(d_1 \mathbf{u}_t + (1-d_1)\begin{pmatrix}0 \\1\end{pmatrix}\big)  \\ & + (1-d_2) \begin{pmatrix}0\\ -1\end{pmatrix}\Big) + 0.05 \omega_t.
\end{align*}
The state space of the collision avoidance environment is define as $\mathcal{X} = [-1,1]^2$. We define the target set as $\Target = [-0.2,0.2]^2$, the initial set $\Init = [-1,-0.9]\times[-0.6,0.6] \cup  [0.9,1.0]\times[-0.6,0.6]$ and the unsafe set $\Unsafe = [-0.3,0.3]\times[0.7,1] \cup  [-0.3,0.3]\times[-1,-0.7]$. Similar to the first two environments, $\omega_t$ is a triangular distributed random variable.

We optimize the training objective using stochastic gradient descent. 
As mentioned in the main text, the policy and RASM networks consist of two hidden layers with 128 units each and ReLU activation function. The RASMs network has single output unit with a softplus activation, while the output dimension of the policy network depends on the task.

The used hyperparameters of our algorithm used in the experiments are listed in Table \ref{tab:hparams}. The code is available for review in the supplementary materials.

\begin{table}[]
    \centering
    \begin{tabular}{c|c}\toprule
    Hyperparameter & Value \\\midrule
         Optimizer & Adam \cite{kingma2014adam} \\
         Batch size & 4096\\
         $V_\nu$ learning rate & 5e-4 \\
    $\pi_\theta$ learning rate & 5e-5 \\
    Lipschitz factor $\gamma$ & 0.001\\
 Lipschitz threshold $\rho_\theta$  & 4\\
  Lipschitz threshold $\rho_\nu$  & 15\\
    $\tau$ (2D system) & 6e-3 \\
  $\tau$ (inverted pendulum) & 2.3e-3 \\
  $\tau$ (collision avoidance) & 4e-3 \\ 
    $\varepsilon$ & 0.3\\
  $N$ & 16 \\
  Number of cells for expectation & 144\\  \bottomrule
    \end{tabular}
    \caption{List of hyperparameter values used in the experiments.}
    \label{tab:hparams}
\end{table}

\textbf{Normalizing the learned RASM for better bounds}

After our algorithm has terminated we can slightly improve the probability bounds certified by the verifier.
In particular, the normalization linearly transforms $V_\nu$ such that the supremum of the new RASM $V'_\nu$ at the initial set is 1 and the infimum of $V'_\nu$ on the entire domain is 0, i.e.,
\begin{equation}
    V'_\nu(\mathbf{x}) = \frac{V_\nu(\mathbf{x})-\inf_{\mathbf{x}' \in \mathcal{X}} V_\nu(\mathbf{x}')}{\sup_{\mathbf{x}' \in \Init} V_\nu(\mathbf{x}')-\inf_{\mathbf{x}' \in \mathcal{X}} V_\nu(\mathbf{x}')}.
\end{equation}
The improved probability bounds $p'$ can then be computed according to condition 3 by 
\begin{equation}
    p' = 1 - \frac{1}{\inf_{\mathbf{x} \in \Unsafe} V'_\nu(\mathbf{x})}.
\end{equation}

The supremum and infimum are computed using our abstract interpretation (IA-AI) on the cell grids.

\textbf{PPO Details}\label{app:ppo}
Here, we list the settings used for the PPO pre-training process of the policy networks \cite{schulman2017proximal}.
In every PPO iteration we collect 30 episodes of the environment as training data in the experience buffer. The policy $\pi_\mu$ is made stochastic using a Gaussian distributed random variable that is added to the policy's output, i.e., the policy predicts the mean of the Gaussian. 
The standard deviation of the Gaussian is annealed during the policy training process, starting from 0.5 at first PPO iteration to 0.05 at PPO iteration 50. We normalize the advantage values, i.e., the difference between the observed discounted returns and the predicted return by the value function, by subtracting the mean and dividing by the standard deviation of the advantage values of the experience buffer. The PPO clipping value $\varepsilon$ is set to 0.2 and the discount factor $\gamma$ to 0.99.
In every PPO iteration, the policy is trained for 10 epochs, except for the first iteration where the network is trained for 30 epochs. An epoch corresponds to a pass over the entire data in the experience buffer, i.e., the data from the the 30 episodes. 
The value network is trained for 5 epochs, expect in the first PPO iteration, where the training is performed for 10 epochs. We apply the Lipschitz regularization on the policy parameters already during the PPO pre-training of the policy.
